How does Software Change?

Software evolves with changes to its codebase over time. Internally, software changes in response to decisions to include some code change into the codebase and discard others. Explaining the mechanism of software evolution, this paper presents a theory of software change. Our theory is grounded in multiple evidence sources (e.g., GitHub documentation and relevant scientific literature) relating to the pull-based development model in GitHub. The resulting theory explains the influence of project-related core concepts (e.g., people and governance) as well as its ecosystem on the decision of software change.

==> Arxiv - A Theory of Software Change (Version 6899)/preprocess.tex <==
\usepackage{xcolor}
\usepackage{tabularx}
\usepackage{flushend}

% Packages for drawing state transition diagram
\usepackage{pgf}
\usepackage{tikz}
\usetikzlibrary{arrows,automata}
\usepackage{verbatim}

\usepackage{arydshln}

\usepackage{cite}
\usepackage{url}
\usepackage{graphicx}
\usepackage{framed}

\graphicspath{{./diagrams/}}

\newcommand{\Se}{Software Engineering}
\newcommand{\se}{software engineering}
\newcommand{\prs}{pull requests}
\newcommand{\td}[1]{{\color{red} TODO: #1}}
\newcommand{\ol}[1]{{\color{purple} Outline: #1}}
\newcommand{\ar}[1]{{\color{blue} Ayushi: #1}}
\newcommand{\gs}[1]{{\color{orange} Georgios: #1}}

==> Arxiv - A Theory of Software Change (Version 6899)/relationsTable.tex <==
%!TEX root =theory.tex
\begin{table*}
\caption{Propositions and explanations derived from the theory of software change}
\label{tab:relationsTable}
\begin{tabularx}{\linewidth}{r X}
\hline
%\multicolumn{2}{l}{Constructs}\\ \hline
%C1 & Available unit changes\\
%C2 & Existing codebase\\
%C3 & People\\
%C4 & Governance \\
%C5 & Tools and technology\\
%C6 & Ecosystem\\
%\hline
\multicolumn{2}{l}{Propositions}\\ 
\hline
%P01 & Characteristics of a unit change influence the decision of software change.\\
\multicolumn{2}{l}{\emph{Investigated in the existing work}}\\
P01 & Unit changes compliant to the project vision are more likely to be integrated into existing codebase. \\
P02 & Unit changes with no dependency to other unit changes are more likely to be integrated into existing codebase. \\
P03 & Larger the impact of unit change; less likely it is to be integrated.\\
P04 & A well-modularized codebase increases the chance of unit change acceptance. \\ 
P05 & Decision to accept unit changes is affected by the signals that maintainers consciously or subconsciously consume through their interactions with contributors. \\
P06 & Tools and technology can improve the quality of a unit change, and therefore its chances of acceptance.\\
\\
\multicolumn{2}{l}{\emph{Emerging from the theory of software change}}\\

P07 & Unit changes that adapt to the technical norms of its ecosystem are more likely to be accepted.\\
P08 & Projects with strong tool support are more likely to scrutinize unit changes more.\\
P09 & Unit changes from new contributors that follow the guidelines are more likely to be accepted. \\
P10 & Unit changes from new contributors originating in the same ecosystem are more likely to be accepted. \\

\hline
\multicolumn{2}{l}{\emph{Explanations}}\\ 
\hline
E01 & Maintainers and stakeholders
% define the project vision and 
need to follow guidelines (e.g., project roadmaps that make project vision explicit) \\
E02 & Unit changes enter the review process; this entails cross-examination of the unit change along with other unit changes. Fewer cross-dependencies facilitate cross-examination. \\
E03 & Syntactic or semantic dependencies of a unit change to existing codebase and its transitive impact complicate the assessment of unit changes. \\
E04 & The impact of a unit change is easier to be assessed on well-architected projects, as their impact is contained. \\
E05 & The characteristics of people participating in the decision process influence the decision.\\
E06 & Automated feedback can improve both the internal quality and the adherence to project guidelines.\\
E07 & A project inherits standards and technical norms from its ecosystem (e.g. dependency declaration files); unit changes not using such standards may break the ecosystem.\\
E08 & Tools improve human abilities by automating repetitive tasks and enabling them to consume more information. Therefore, maintainers are better equipped to investigate unit changes in depth.\\
E09 & As trust between the contributor and the maintainer can not be established otherwise, adherence to guidelines is a signal for quality.\\
E10 & Trust is established by examining contributor profile within a set of interrelated projects. \\

\hline
%\multicolumn{2}{l}{Scope}\\ 
%\hline
% & Theory of software change explains evolution of a software system from a given state to the next. 
%On reaching the next stage, recursive effects on the elements of software change begin, which are not a part of this theory. 
%This theory is derived from and applies to collaboratively developed software projects developed in open source. 
%Although the theory is likely to be applicable in commercial software projects too.
%\\ \hline
\end{tabularx}
\end{table*}
